Generative Graphical Inverse Kinematics

Quickly and reliably finding accurate inverse kinematics (IK) solutions remains a challenging problem for many robot manipulators. Existing numerical solvers are broadly applicable but typically only produce a single solution and rely on local search techniques to minimize nonconvex objective functions. More recent learning-based approaches that approximate the entire feasible set of solutions have shown promise as a means to generate multiple fast and accurate IK results in parallel. However, existing learning-based techniques have a significant drawback: each robot of interest requires a specialized model that must be trained from scratch. To address this key shortcoming, we propose a novel distance-geometric robot representation coupled with a graph structure that allows us to leverage the sample efficiency of Euclidean equivariant functions and the generalizability of graph neural networks (GNNs). Our approach is generative graphical inverse kinematics (GGIK), the first learned IK solver able to accurately and efficiently produce a large number of diverse solutions in parallel while also displaying the ability to generalize -- a single learned model can be used to produce IK solutions for a variety of different robots. When compared to several other learned IK methods, GGIK provides more accurate solutions with the same amount of data. GGIK can generalize reasonably well to robot manipulators unseen during training. Additionally, GGIK can learn a constrained distribution that encodes joint limits and scales efficiently to larger robots and a high number of sampled solutions. Finally, GGIK can be used to complement local IK solvers by providing reliable initializations for a local optimization process.

==> figures/tikz/timing_plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{gray14712096}{RGB}{147,120,96}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lavender234234242}{RGB}{234,234,242}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightslategray129114179}{RGB}{129,114,179}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis background/.style={fill=lavender234234242},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204,
  fill=lavender234234242
},
tick align=outside,
x grid style={white},
xlabel=\textcolor{darkslategray38}{Number of samples},
xmajorgrids,
xmajorticks=false,
xmajorticks=true,
xmin=-50.15, xmax=1075.15,
xtick pos=left,
xtick style={color=darkslategray38},
xtick={-200,0,200,400,600,800,1000,1200},
xticklabels={
  \(\displaystyle {\ensuremath{-}200}\),
  \(\displaystyle {0}\),
  \(\displaystyle {200}\),
  \(\displaystyle {400}\),
  \(\displaystyle {600}\),
  \(\displaystyle {800}\),
  \(\displaystyle {1000}\),
  \(\displaystyle {1200}\)
},
y grid style={white},
ylabel=\textcolor{darkslategray38}{Time [s]},
ymajorgrids,
ymajorticks=false,
ymajorticks=true,
ymin=-0.0608289705572258, ymax=1.31552994036231,
ytick pos=left,
ytick style={color=darkslategray38},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2,1.4},
yticklabels={
  \(\displaystyle {\ensuremath{-}0.2}\),
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.8}\),
  \(\displaystyle {1.0}\),
  \(\displaystyle {1.2}\),
  \(\displaystyle {1.4}\)
}
]
\path [draw=steelblue76114176, fill=steelblue76114176, opacity=0.2]
(axis cs:1,0.00772555871641852)
--(axis cs:1,0.00725332693421624)
--(axis cs:16,0.00757752053310052)
--(axis cs:64,0.00977572365410794)
--(axis cs:128,0.0127913753620339)
--(axis cs:256,0.020525615074215)
--(axis cs:512,0.0362105510277068)
--(axis cs:1024,0.0436125018154863)
--(axis cs:1024,0.108762838646245)
--(axis cs:1024,0.108762838646245)
--(axis cs:512,0.0365269937473023)
--(axis cs:256,0.0212809039573096)
--(axis cs:128,0.0131731529601859)
--(axis cs:64,0.00982788638464938)
--(axis cs:16,0.00764458187054022)
--(axis cs:1,0.00772555871641852)
--cycle;

\path [draw=peru22113282, fill=peru22113282, opacity=0.2]
(axis cs:1,0.00757987964250857)
--(axis cs:1,0.00753114950559323)
--(axis cs:16,0.00833030936547571)
--(axis cs:64,0.0173094252512907)
--(axis cs:128,0.0254350642795692)
--(axis cs:256,0.0457972612999212)
--(axis cs:512,0.0870269937966095)
--(axis cs:1024,0.17084719568985)
--(axis cs:1024,0.171304803783721)
--(axis cs:1024,0.171304803783721)
--(axis cs:512,0.0872502223994507)
--(axis cs:256,0.0460193726398219)
--(axis cs:128,0.0257198770408501)
--(axis cs:64,0.0175825079514528)
--(axis cs:16,0.00850275757483191)
--(axis cs:1,0.00757987964250857)
--cycle;

\path [draw=mediumseagreen85168104, fill=mediumseagreen85168104, opacity=0.2]
(axis cs:1,0.00773413048006861)
--(axis cs:1,0.00745107664845617)
--(axis cs:16,0.011361266902921)
--(axis cs:64,0.0284282476963715)
--(axis cs:128,0.0444999193494459)
--(axis cs:256,0.0845208369316137)
--(axis cs:512,0.166671405585082)
--(axis cs:1024,0.331882238832724)
--(axis cs:1024,0.333395450862634)
--(axis cs:1024,0.333395450862634)
--(axis cs:512,0.166957397906511)
--(axis cs:256,0.0851542152343714)
--(axis cs:128,0.0450762057955126)
--(axis cs:64,0.0289663164553924)
--(axis cs:16,0.0117044491252925)
--(axis cs:1,0.00773413048006861)
--cycle;

\path [draw=indianred1967882, fill=indianred1967882, opacity=0.2]
(axis cs:1,0.00832957379620318)
--(axis cs:1,0.00713842756945844)
--(axis cs:16,0.0151746463894488)
--(axis cs:64,0.0419478340206487)
--(axis cs:128,0.0710095582781908)
--(axis cs:256,0.137446580196065)
--(axis cs:512,0.273340289026072)
--(axis cs:1024,0.522221086282234)
--(axis cs:1024,0.523611100655098)
--(axis cs:1024,0.523611100655098)
--(axis cs:512,0.27482333359165)
--(axis cs:256,0.137946786617595)
--(axis cs:128,0.0713557185353163)
--(axis cs:64,0.0432577805461543)
--(axis cs:16,0.0155081558108685)
--(axis cs:1,0.00832957379620318)
--cycle;

\path [draw=lightslategray129114179, fill=lightslategray129114179, opacity=0.2]
(axis cs:1,0.00771206875493622)
--(axis cs:1,0.00748431424448394)
--(axis cs:16,0.0200489704525584)
--(axis cs:64,0.0534444592798502)
--(axis cs:128,0.103822893389044)
--(axis cs:256,0.205057697731318)
--(axis cs:512,0.411642528489714)
--(axis cs:1024,0.765465629594916)
--(axis cs:1024,0.826633411151773)
--(axis cs:1024,0.826633411151773)
--(axis cs:512,0.412829600855226)
--(axis cs:256,0.205741924804387)
--(axis cs:128,0.105061375610055)
--(axis cs:64,0.0576175309812277)
--(axis cs:16,0.0201917345607167)
--(axis cs:1,0.00771206875493622)
--cycle;

\path [draw=gray14712096, fill=gray14712096, opacity=0.2]
(axis cs:1,0.0076469573307732)
--(axis cs:1,0.00753041178696361)
--(axis cs:16,0.00173279812093482)
--(axis cs:64,0.0741618762949665)
--(axis cs:128,0.145026948947236)
--(axis cs:256,0.286793334167628)
--(axis cs:512,0.547294849559003)
--(axis cs:1024,1.03296380296528)
--(axis cs:1024,1.25296817168415)
--(axis cs:1024,1.25296817168415)
--(axis cs:512,0.549251532152957)
--(axis cs:256,0.289461063463064)
--(axis cs:128,0.145557853680328)
--(axis cs:64,0.0743731667062084)
--(axis cs:16,0.0666744096064974)
--(axis cs:1,0.0076469573307732)
--cycle;

\addplot [semithick, steelblue76114176, forget plot]
table {%
1 0.00748944282531738
16 0.00761105120182037
64 0.00980180501937866
128 0.0129822641611099
256 0.0209032595157623
512 0.0363687723875046
1024 0.0761876702308655
};
\addplot [semithick, peru22113282, forget plot]
table {%
1 0.0075555145740509
16 0.00841653347015381
64 0.0174459666013718
128 0.0255774706602097
256 0.0459083169698715
512 0.0871386080980301
1024 0.171075999736786
};
\addplot [semithick, mediumseagreen85168104, forget plot]
table {%
1 0.00759260356426239
16 0.0115328580141068
64 0.028697282075882
128 0.0447880625724792
256 0.0848375260829926
512 0.166814401745796
1024 0.332638844847679
};
\addplot [semithick, indianred1967882, forget plot]
table {%
1 0.00773400068283081
16 0.0153414011001587
64 0.0426028072834015
128 0.0711826384067535
256 0.13769668340683
512 0.274081811308861
1024 0.522916093468666
};
\addplot [semithick, lightslategray129114179, forget plot]
table {%
1 0.00759819149971008
16 0.0201203525066376
64 0.0555309951305389
128 0.10444213449955
256 0.205399811267853
512 0.41223606467247
1024 0.796049520373344
};
\addplot [semithick, gray14712096, forget plot]
table {%
1 0.00758868455886841
16 0.0342036038637161
64 0.0742675215005875
128 0.145292401313782
256 0.288127198815346
512 0.54827319085598
1024 1.14296598732471
};
\end{axis}



==> tables/experiment_1.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & Success [\%] \\
 & mean & min & 25\% & 50\% & 75\% & mean & min & 25\% & 50\% & 75\% &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
4 & 17.7 & 3.8 & 10.1 & 14.4 & 20.7 & 2.6 & 0.4 & 1.6 & 2.4 & 3.4 & 93.2 \\
5 & 23.3 & 3.8 & 11.3 & 16.4 & 25.3 & 2.2 & 0.4 & 1.3 & 2.1 & 2.9 & 94.0 \\
6 & 29.9 & 5.4 & 15.2 & 22.2 & 34.7 & 2.2 & 0.4 & 1.3 & 2.1 & 3.0 & 88.0 \\
7 & 38.7 & 7.0 & 20.9 & 31.3 & 48.5 & 2.6 & 0.5 & 1.5 & 2.4 & 3.4 & 81.8 \\
8 & 81.7 & 13.9 & 48.1 & 74.5 & 107.7 & 3.8 & 1.1 & 2.5 & 3.6 & 4.8 & 37.0 \\
\bottomrule
\end{tabular}


==> tables/experiment_2.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & Success [\%] \\
 & mean & min & 25\% & 50\% & 75\% & mean & min & 25\% & 50\% & 75\% &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 16.9 & 3.3 & 8.0 & 11.5 & 17.5 & 1.7 & 0.4 & 0.9 & 1.2 & 1.8 & 98.2 \\
lwa4d & 13.6 & 2.7 & 6.5 & 9.6 & 14.5 & 1.9 & 0.4 & 1.0 & 1.4 & 2.0 & 99.2 \\
lwa4p & 7.0 & 2.8 & 5.0 & 6.6 & 8.5 & 2.1 & 1.4 & 1.7 & 2.0 & 2.3 & 97.5 \\
panda & 36.4 & 4.7 & 14.5 & 25.1 & 44.4 & 4.5 & 1.3 & 2.4 & 3.4 & 5.3 & 95.2 \\
ur10 & 17.1 & 5.3 & 10.2 & 14.9 & 21.4 & 1.8 & 0.9 & 1.4 & 1.7 & 2.1 & 89.2 \\
\bottomrule
\end{tabular}


==> tables/experiment_3_local.tex <==
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
 Initialization & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & Success [\%] & Num. Iter. \\
  & mean & min & \edit{Q$_1$} & \edit{Q$_2$} & \edit{Q$_3$} & mean & min & \edit{Q$_1$} & \edit{Q$_2$} & \edit{Q$_3$} &  &  \\
\midrule
Random & 3.8 & 0.0 & 0.2 & 1.4 & 6.3 & 0.04 & 0.0 & 0.0 & 0.0 & 0.04 & 99.9 & 28.7 \\
GGIK & 1.0 & 0.0 & 0.3 & 0.7 & 1.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 99.9 & 11.1 \\
\bottomrule
\end{tabular}

==> tables/experiment_3_ref.tex <==
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & Success [\%] & Num. Iter. \\
 & mean & min & 25\% & 50\% & 75\% & mean & min & 25\% & 50\% & 75\% &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.7 & 0.1 & 0.3 & 0.5 & 0.9 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 100.0 & 10.7 \\
lwa4d & 0.8 & 0.1 & 0.3 & 0.6 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 100.0 & 10.9 \\
lwa4p & 1.2 & 0.3 & 0.7 & 1.0 & 1.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 99.8 & 9.6 \\
panda & 1.0 & 0.0 & 0.1 & 0.4 & 1.3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 100.0 & 14.2 \\
ur10 & 1.5 & 0.2 & 0.3 & 1.0 & 2.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 99.8 & 10.2 \\
\bottomrule
\end{tabular}


==> tables/experiment_3b.tex <==
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
 Robot & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & Success [\%] & MMD\\
 & mean & min & max & Q$_{1}$ & Q$_{3}$ & mean & min & max & Q$_{1}$ & Q$_{3}$ &  & \\
\midrule
kuka & 3.7 & 2.8 & 5.2 & 3.4 & 3.9 & 0.7 & 0.5 & 1.0 & 0.6 & 0.7 & 99.8 & - \\
lwa4d & 3.6 & 2.7 & 5.4 & 3.3 & 3.9 & 0.6 & 0.4 & 0.9 & 0.5 & 0.6 & 99.8 & - \\
lwa4p & 3.8 & 2.7 & 4.9 & 3.4 & 4.1 & 0.5 & 0.3 & 0.7 & 0.4 & 0.6 & 99.5 & - \\
panda & 8.5 & 4.7 & 15.7 & 6.0 & 11.4 & 1.0 & 0.6 & 1.7 & 0.7 & 1.2 & 94.2 & - \\
ur10 & 6.0 & 4.2 & 8.6 & 5.2 & 6.8 & 0.5 & 0.4 & 0.8 & 0.5 & 0.6 & 97.2 & - \\
\bottomrule
\end{tabular}


==> tables/experiment_panda.tex <==
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
 Robot & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & MMD & Success [\%] \\
 & mean & min & max & Q$_{1}$ & Q$_{3}$ & mean & min & max & Q$_{1}$ & Q$_{3}$ &  \\
\midrule
GGIK & 3.0 & 2.2 & 5.0 & 2.7 & 3.2 & 0.4 & 0.3 & 0.7 & 0.4 & 0.4 & .08 & 99.8 \\
IKFlow & 7.72 & - & - & - & - & 2.81 & - & - & - & - & .03 & - \\
\bottomrule
\end{tabular}

==> tables/tracik_ggik.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 25.5 & 0.0 & 0.0 & 0.0 & 1378.0 & 1.9 & 0.0 & 0.0 & 0.0 & 124.4 & 0.0 & 0.0 & 20.7 & 139.7 & 98.0 & TRACIK + GGIK \\
lwa4d & 5.9 & 0.0 & 0.0 & 0.0 & 1428.0 & 0.7 & 0.0 & 0.0 & 0.0 & 127.5 & 0.0 & 0.0 & 13.9 & 95.3 & 99.4 & TRACIK + GGIK \\
lwa4p & 1.2 & 0.0 & 0.0 & 0.0 & 948.8 & 0.2 & 0.0 & 0.0 & 0.0 & 122.2 & 0.0 & 0.0 & 11.3 & 57.6 & 99.8 & TRACIK + GGIK \\
panda & 185.4 & 0.0 & 0.0 & 0.0 & 1433.4 & 17.0 & 0.0 & 0.0 & 0.0 & 135.6 & 0.0 & 0.0 & 174.2 & 377.5 & 82.7 & TRACIK + GGIK \\
ur10 & 1.1 & 0.0 & 0.0 & 0.0 & 847.7 & 0.2 & 0.0 & 0.0 & 0.0 & 125.1 & 0.0 & 0.0 & 2.8 & 37.0 & 99.9 & TRACIK + GGIK \\
\bottomrule
\end{tabular}


==> tables/tracik_random.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 25.5 & 0.0 & 0.0 & 0.0 & 1378.0 & 1.9 & 0.0 & 0.0 & 0.0 & 124.4 & 0.0 & 0.0 & 20.8 & 139.7 & 98.0 & TRACIK + rand \\
lwa4d & 5.9 & 0.0 & 0.0 & 0.0 & 1428.0 & 0.6 & 0.0 & 0.0 & 0.0 & 129.5 & 0.0 & 0.0 & 13.8 & 94.5 & 99.4 & TRACIK + rand \\
lwa4p & 1.2 & 0.0 & 0.0 & 0.0 & 948.8 & 0.2 & 0.0 & 0.0 & 0.0 & 122.2 & 0.0 & 0.0 & 13.4 & 64.5 & 99.9 & TRACIK + rand \\
panda & 182.2 & 0.0 & 0.0 & 0.0 & 1397.4 & 16.8 & 0.0 & 0.0 & 0.0 & 134.7 & 0.0 & 0.0 & 171.9 & 375.3 & 83.0 & TRACIK + rand \\
ur10 & 1.3 & 0.0 & 0.0 & 0.0 & 847.7 & 0.3 & 0.0 & 0.0 & 0.0 & 125.1 & 0.0 & 0.0 & 3.4 & 37.9 & 99.7 & TRACIK + rand \\
\bottomrule
\end{tabular}


==> tables/tracik_tables_per_method.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  \\
Initialization &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
GGIK & 14.8 & 1.0 & 6.5 & 17.8 & 94.9 & 1.5 & 0.0 & 0.6 & 1.7 & 22.7 & 1.0 & 0.0 & 9.2 & 0.3 & 53.6 \\
SQP + rand & 1.6 & 0.0 & 0.1 & 0.2 & 67.7 & 0.0 & 0.0 & 0.0 & 0.0 & 0.4 & 29.5 & 11.5 & 98.4 & 38.8 & 96.0 \\
SQP + GGIK & 0.8 & 0.0 & 0.1 & 0.7 & 12.6 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 11.2 & 4.6 & 38.0 & 13.4 & 99.5 \\
GRAPHIK + rand & 32.0 & 0.0 & 20.8 & 39.2 & 223.3 & 1.8 & 0.0 & 1.0 & 2.1 & 14.4 & 182.3 & 144.3 & 261.9 & 232.1 & 79.2 \\
GRAPHIK + GGIK & 0.3 & 0.0 & 0.1 & 0.2 & 30.4 & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 87.3 & 111.9 & 180.2 & 217.7 & 99.5 \\
TRACIK + rand & 43.2 & 0.0 & 0.0 & 0.0 & 1200.0 & 3.9 & 0.0 & 0.0 & 0.0 & 127.2 & 0.0 & 0.0 & 44.6 & 142.4 & 96.0 \\
TRACIK + GGIK & 43.8 & 0.0 & 0.0 & 0.0 & 1207.2 & 4.0 & 0.0 & 0.0 & 0.0 & 126.9 & 0.0 & 0.0 & 44.6 & 141.4 & 95.9 \\
\bottomrule
\end{tabular}


==> tables/tracik_tables_per_robot.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 13.4 & 0.9 & 6.4 & 15.6 & 102.5 & 1.6 & 0.0 & 0.6 & 1.6 & 26.7 & 1.0 & 0.0 & 9.3 & 0.5 & 50.0 & GGIK \\
lwa4d & 11.3 & 0.6 & 5.8 & 12.7 & 105.8 & 1.5 & 0.0 & 0.7 & 1.7 & 21.4 & 1.0 & 0.0 & 9.3 & 0.4 & 58.9 & GGIK \\
lwa4p & 6.7 & 0.6 & 3.7 & 8.0 & 52.0 & 1.0 & 0.0 & 0.4 & 1.0 & 25.5 & 1.0 & 0.0 & 9.2 & 0.3 & 87.2 & GGIK \\
panda & 26.6 & 1.4 & 10.5 & 35.1 & 110.7 & 2.4 & 0.0 & 0.8 & 2.8 & 22.8 & 1.0 & 0.0 & 9.1 & 0.2 & 23.5 & GGIK \\
ur10 & 15.8 & 1.2 & 6.4 & 17.4 & 103.6 & 1.1 & 0.0 & 0.5 & 1.2 & 16.9 & 1.0 & 0.0 & 9.1 & 0.2 & 48.4 & GGIK \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.6 & 0.0 & 0.1 & 0.2 & 42.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 29.4 & 12.6 & 104.6 & 45.8 & 98.4 & SQP + rand \\
lwa4d & 1.3 & 0.0 & 0.1 & 0.2 & 76.3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.4 & 31.2 & 12.1 & 109.2 & 43.2 & 96.6 & SQP + rand \\
lwa4p & 2.0 & 0.0 & 0.1 & 0.2 & 59.8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 31.6 & 12.6 & 95.6 & 39.2 & 93.6 & SQP + rand \\
panda & 2.6 & 0.0 & 0.1 & 0.2 & 81.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 32.2 & 12.6 & 111.5 & 43.4 & 94.5 & SQP + rand \\
ur10 & 1.4 & 0.0 & 0.0 & 0.1 & 79.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 23.1 & 7.4 & 71.2 & 22.2 & 96.7 & SQP + rand \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.7 & 0.0 & 0.1 & 0.6 & 11.8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 11.0 & 4.4 & 40.0 & 13.4 & 99.6 & SQP + GGIK \\
lwa4d & 0.8 & 0.0 & 0.1 & 1.0 & 13.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 10.6 & 4.6 & 38.3 & 13.9 & 99.7 & SQP + GGIK \\
lwa4p & 1.0 & 0.0 & 0.2 & 1.2 & 12.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 9.8 & 3.9 & 31.2 & 10.5 & 99.4 & SQP + GGIK \\
panda & 0.6 & 0.0 & 0.1 & 0.3 & 12.6 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 14.0 & 6.3 & 48.3 & 19.2 & 99.9 & SQP + GGIK \\
ur10 & 0.6 & 0.0 & 0.1 & 0.5 & 12.9 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 10.3 & 3.6 & 32.4 & 9.9 & 99.1 & SQP + GGIK \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.4 & 0.0 & 0.1 & 0.2 & 15.7 & 0.0 & 0.0 & 0.0 & 0.0 & 1.2 & 208.6 & 147.8 & 345.4 & 258.8 & 99.4 & GRAPHIK + rand \\
lwa4d & 2.0 & 0.0 & 0.1 & 0.3 & 281.2 & 0.1 & 0.0 & 0.0 & 0.0 & 17.2 & 203.2 & 154.0 & 301.1 & 253.8 & 98.5 & GRAPHIK + rand \\
lwa4p & 7.9 & 0.0 & 0.1 & 0.3 & 282.1 & 0.6 & 0.0 & 0.0 & 0.0 & 17.6 & 242.1 & 181.8 & 343.8 & 291.7 & 92.0 & GRAPHIK + rand \\
panda & 139.0 & 0.0 & 103.6 & 194.7 & 293.2 & 7.8 & 0.0 & 4.7 & 10.4 & 17.9 & 78.1 & 71.8 & 62.9 & 96.9 & 16.2 & GRAPHIK + rand \\
ur10 & 10.6 & 0.0 & 0.1 & 0.3 & 244.0 & 0.8 & 0.0 & 0.0 & 0.0 & 18.0 & 179.4 & 166.3 & 256.2 & 259.3 & 89.8 & GRAPHIK + rand \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.2 & 0.0 & 0.1 & 0.2 & 9.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.6 & 112.7 & 130.4 & 258.9 & 272.2 & 100.0 & GRAPHIK + GGIK \\
lwa4d & 0.3 & 0.0 & 0.1 & 0.2 & 30.7 & 0.0 & 0.0 & 0.0 & 0.0 & 2.0 & 100.6 & 135.4 & 207.2 & 264.4 & 99.6 & GRAPHIK + GGIK \\
lwa4p & 0.4 & 0.0 & 0.1 & 0.3 & 45.8 & 0.0 & 0.0 & 0.0 & 0.0 & 3.2 & 122.6 & 153.5 & 246.5 & 296.0 & 99.5 & GRAPHIK + GGIK \\
panda & 0.1 & 0.0 & 0.0 & 0.0 & 27.6 & 0.0 & 0.0 & 0.0 & 0.0 & 1.6 & 27.9 & 45.6 & 35.9 & 66.5 & 99.9 & GRAPHIK + GGIK \\
ur10 & 0.6 & 0.0 & 0.1 & 0.2 & 38.5 & 0.0 & 0.0 & 0.0 & 0.0 & 3.4 & 72.5 & 94.6 & 152.6 & 189.4 & 98.4 & GRAPHIK + GGIK \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 25.5 & 0.0 & 0.0 & 0.0 & 1378.0 & 1.9 & 0.0 & 0.0 & 0.0 & 124.4 & 0.0 & 0.0 & 20.8 & 139.7 & 98.0 & TRACIK + rand \\
lwa4d & 5.9 & 0.0 & 0.0 & 0.0 & 1428.0 & 0.6 & 0.0 & 0.0 & 0.0 & 129.5 & 0.0 & 0.0 & 13.8 & 94.5 & 99.4 & TRACIK + rand \\
lwa4p & 1.2 & 0.0 & 0.0 & 0.0 & 948.8 & 0.2 & 0.0 & 0.0 & 0.0 & 122.2 & 0.0 & 0.0 & 13.4 & 64.5 & 99.9 & TRACIK + rand \\
panda & 182.2 & 0.0 & 0.0 & 0.0 & 1397.4 & 16.8 & 0.0 & 0.0 & 0.0 & 134.7 & 0.0 & 0.0 & 171.9 & 375.3 & 83.0 & TRACIK + rand \\
ur10 & 1.3 & 0.0 & 0.0 & 0.0 & 847.7 & 0.3 & 0.0 & 0.0 & 0.0 & 125.1 & 0.0 & 0.0 & 3.4 & 37.9 & 99.7 & TRACIK + rand \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 25.5 & 0.0 & 0.0 & 0.0 & 1378.0 & 1.9 & 0.0 & 0.0 & 0.0 & 124.4 & 0.0 & 0.0 & 20.7 & 139.7 & 98.0 & TRACIK + GGIK \\
lwa4d & 5.9 & 0.0 & 0.0 & 0.0 & 1428.0 & 0.7 & 0.0 & 0.0 & 0.0 & 127.5 & 0.0 & 0.0 & 13.9 & 95.3 & 99.4 & TRACIK + GGIK \\
lwa4p & 1.2 & 0.0 & 0.0 & 0.0 & 948.8 & 0.2 & 0.0 & 0.0 & 0.0 & 122.2 & 0.0 & 0.0 & 11.3 & 57.6 & 99.8 & TRACIK + GGIK \\
panda & 185.4 & 0.0 & 0.0 & 0.0 & 1433.4 & 17.0 & 0.0 & 0.0 & 0.0 & 135.6 & 0.0 & 0.0 & 174.2 & 377.5 & 82.7 & TRACIK + GGIK \\
ur10 & 1.1 & 0.0 & 0.0 & 0.0 & 847.7 & 0.2 & 0.0 & 0.0 & 0.0 & 125.1 & 0.0 & 0.0 & 2.8 & 37.0 & 99.9 & TRACIK + GGIK \\
\bottomrule
\end{tabular}


==> tables/tracik_tables_per_robot_original.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
 Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 13.4 & 0.9 & 6.4 & 15.6 & 102.5 & 1.6 & 0.0 & 0.6 & 1.6 & 26.7 & 1.0 & 0.0 & 9.3 & 0.5 & 50.0 & GGIK \\
lwa4d & 11.3 & 0.6 & 5.8 & 12.7 & 105.8 & 1.5 & 0.0 & 0.7 & 1.7 & 21.4 & 1.0 & 0.0 & 9.3 & 0.4 & 58.9 & GGIK \\
lwa4p & 6.7 & 0.6 & 3.7 & 8.0 & 52.0 & 1.0 & 0.0 & 0.4 & 1.0 & 25.5 & 1.0 & 0.0 & 9.2 & 0.3 & 87.2 & GGIK \\
panda & 26.6 & 1.4 & 10.5 & 35.1 & 110.7 & 2.4 & 0.0 & 0.8 & 2.8 & 22.8 & 1.0 & 0.0 & 9.1 & 0.2 & 23.5 & GGIK \\
ur10 & 15.8 & 1.2 & 6.4 & 17.4 & 103.6 & 1.1 & 0.0 & 0.5 & 1.2 & 16.9 & 1.0 & 0.0 & 9.1 & 0.2 & 48.4 & GGIK \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.6 & 0.0 & 0.1 & 0.2 & 42.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 29.4 & 12.6 & 104.6 & 45.8 & 98.4 & SQP + rand \\
lwa4d & 1.3 & 0.0 & 0.1 & 0.2 & 76.3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.4 & 31.2 & 12.1 & 109.2 & 43.2 & 96.6 & SQP + rand \\
lwa4p & 2.0 & 0.0 & 0.1 & 0.2 & 59.8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.3 & 31.6 & 12.6 & 95.6 & 39.2 & 93.6 & SQP + rand \\
panda & 2.6 & 0.0 & 0.1 & 0.2 & 81.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 32.2 & 12.6 & 111.5 & 43.4 & 94.5 & SQP + rand \\
ur10 & 1.4 & 0.0 & 0.0 & 0.1 & 79.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 23.1 & 7.4 & 71.2 & 22.2 & 96.7 & SQP + rand \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.7 & 0.0 & 0.1 & 0.6 & 11.8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 11.0 & 4.4 & 40.0 & 13.4 & 99.6 & SQP + GGIK \\
lwa4d & 0.8 & 0.0 & 0.1 & 1.0 & 13.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 10.6 & 4.6 & 38.3 & 13.9 & 99.7 & SQP + GGIK \\
lwa4p & 1.0 & 0.0 & 0.2 & 1.2 & 12.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 9.8 & 3.9 & 31.2 & 10.5 & 99.4 & SQP + GGIK \\
panda & 0.6 & 0.0 & 0.1 & 0.3 & 12.6 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 14.0 & 6.3 & 48.3 & 19.2 & 99.9 & SQP + GGIK \\
ur10 & 0.6 & 0.0 & 0.1 & 0.5 & 12.9 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 10.3 & 3.6 & 32.4 & 9.9 & 99.1 & SQP + GGIK \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.4 & 0.0 & 0.1 & 0.2 & 15.7 & 0.0 & 0.0 & 0.0 & 0.0 & 1.2 & 208.6 & 147.8 & 345.4 & 258.8 & 99.4 & GRAPHIK + rand \\
lwa4d & 2.0 & 0.0 & 0.1 & 0.3 & 281.2 & 0.1 & 0.0 & 0.0 & 0.0 & 17.2 & 203.2 & 154.0 & 301.1 & 253.8 & 98.5 & GRAPHIK + rand \\
lwa4p & 7.9 & 0.0 & 0.1 & 0.3 & 282.1 & 0.6 & 0.0 & 0.0 & 0.0 & 17.6 & 242.1 & 181.8 & 343.8 & 291.7 & 92.0 & GRAPHIK + rand \\
panda & 139.0 & 0.0 & 103.6 & 194.7 & 293.2 & 7.8 & 0.0 & 4.7 & 10.4 & 17.9 & 78.1 & 71.8 & 62.9 & 96.9 & 16.2 & GRAPHIK + rand \\
ur10 & 10.6 & 0.0 & 0.1 & 0.3 & 244.0 & 0.8 & 0.0 & 0.0 & 0.0 & 18.0 & 179.4 & 166.3 & 256.2 & 259.3 & 89.8 & GRAPHIK + rand \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 0.2 & 0.0 & 0.1 & 0.2 & 9.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.6 & 112.7 & 130.4 & 258.9 & 272.2 & 100.0 & GRAPHIK + GGIK \\
lwa4d & 0.3 & 0.0 & 0.1 & 0.2 & 30.7 & 0.0 & 0.0 & 0.0 & 0.0 & 2.0 & 100.6 & 135.4 & 207.2 & 264.4 & 99.6 & GRAPHIK + GGIK \\
lwa4p & 0.4 & 0.0 & 0.1 & 0.3 & 45.8 & 0.0 & 0.0 & 0.0 & 0.0 & 3.2 & 122.6 & 153.5 & 246.5 & 296.0 & 99.5 & GRAPHIK + GGIK \\
panda & 0.1 & 0.0 & 0.0 & 0.0 & 27.6 & 0.0 & 0.0 & 0.0 & 0.0 & 1.6 & 27.9 & 45.6 & 35.9 & 66.5 & 99.9 & GRAPHIK + GGIK \\
ur10 & 0.6 & 0.0 & 0.1 & 0.2 & 38.5 & 0.0 & 0.0 & 0.0 & 0.0 & 3.4 & 72.5 & 94.6 & 152.6 & 189.4 & 98.4 & GRAPHIK + GGIK \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 25.5 & 0.0 & 0.0 & 0.0 & 1378.0 & 1.9 & 0.0 & 0.0 & 0.0 & 124.4 & 0.0 & 0.0 & 20.8 & 139.7 & 98.0 & TRACIK + rand \\
lwa4d & 5.9 & 0.0 & 0.0 & 0.0 & 1428.0 & 0.6 & 0.0 & 0.0 & 0.0 & 129.5 & 0.0 & 0.0 & 13.8 & 94.5 & 99.4 & TRACIK + rand \\
lwa4p & 1.2 & 0.0 & 0.0 & 0.0 & 948.8 & 0.2 & 0.0 & 0.0 & 0.0 & 122.2 & 0.0 & 0.0 & 13.4 & 64.5 & 99.9 & TRACIK + rand \\
panda & 182.2 & 0.0 & 0.0 & 0.0 & 1397.4 & 16.8 & 0.0 & 0.0 & 0.0 & 134.7 & 0.0 & 0.0 & 171.9 & 375.3 & 83.0 & TRACIK + rand \\
ur10 & 1.3 & 0.0 & 0.0 & 0.0 & 847.7 & 0.3 & 0.0 & 0.0 & 0.0 & 125.1 & 0.0 & 0.0 & 3.4 & 37.9 & 99.7 & TRACIK + rand \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrrrrrrrrl}
\toprule
 & \multicolumn{5}{c}{Err. Pos. [mm]} & \multicolumn{5}{c}{Err. Rot. [deg]} & \multicolumn{2}{c}{Num. Iter.} & \multicolumn{2}{c}{Time [ms]} & Success [\%] & Initialization \\
 & mean & min & 25\% & 75\% & max & mean & min & 25\% & 75\% & max & mean & std & mean & std &  &  \\
Robot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
kuka & 25.5 & 0.0 & 0.0 & 0.0 & 1378.0 & 1.9 & 0.0 & 0.0 & 0.0 & 124.4 & 0.0 & 0.0 & 20.7 & 139.7 & 98.0 & TRACIK + GGIK \\
lwa4d & 5.9 & 0.0 & 0.0 & 0.0 & 1428.0 & 0.7 & 0.0 & 0.0 & 0.0 & 127.5 & 0.0 & 0.0 & 13.9 & 95.3 & 99.4 & TRACIK + GGIK \\
lwa4p & 1.2 & 0.0 & 0.0 & 0.0 & 948.8 & 0.2 & 0.0 & 0.0 & 0.0 & 122.2 & 0.0 & 0.0 & 11.3 & 57.6 & 99.8 & TRACIK + GGIK \\
panda & 185.4 & 0.0 & 0.0 & 0.0 & 1433.4 & 17.0 & 0.0 & 0.0 & 0.0 & 135.6 & 0.0 & 0.0 & 174.2 & 377.5 & 82.7 & TRACIK + GGIK \\
ur10 & 1.1 & 0.0 & 0.0 & 0.0 & 847.7 & 0.2 & 0.0 & 0.0 & 0.0 & 125.1 & 0.0 & 0.0 & 2.8 & 37.0 & 99.9 & TRACIK + GGIK \\
\bottomrule
\end{tabular}

